An Exponential Lower Bound on OBDD Refutations for Pigeonhole Formulas

Haken proved that every resolution refutation of the pigeonhole formula has at least exponential size. Groote and Zantema proved that a particular OBDD computation of the pigeonhole formula has an exponential size. Here we show that any arbitrary OBDD refutation of the pigeonhole formula has an exponential size, too: we prove that the size of one of the intermediate OBDDs is at least $\Omega(1.025^n)$.

==> eptcsdata.tex <==
\providecommand{\event}{E. Markakis, I. Milis (Eds.): 4th Athens Colloquium\\ 
on Algorithms and Complexity (ACAC 2009)}
\providecommand{\volume}{4}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{13}
\providecommand{\eid}{2}

